Scalable Communication Endpoints for MPI+Threads Applications

Hybrid MPI+threads programming is gaining prominence as an alternative to the traditional "MPI everywhere'" model to better handle the disproportionate increase in the number of cores compared with other on-node resources. Current implementations of these two models represent the two extreme cases of communication resource sharing in modern MPI implementations. In the MPI-everywhere model, each MPI process has a dedicated set of communication resources (also known as endpoints), which is ideal for performance but is resource wasteful. With MPI+threads, current MPI implementations share a single communication endpoint for all threads, which is ideal for resource usage but is hurtful for performance. In this paper, we explore the tradeoff space between performance and communication resource usage in MPI+threads environments. We first demonstrate the two extreme cases---one where all threads share a single communication endpoint and another where each thread gets its own dedicated communication endpoint (similar to the MPI-everywhere model) and showcase the inefficiencies in both these cases. Next, we perform a thorough analysis of the different levels of resource sharing in the context of Mellanox InfiniBand. Using the lessons learned from this analysis, we design an improved resource-sharing model to produce \emph{scalable communication endpoints} that can achieve the same performance as with dedicated communication resources per thread but using just a third of the resources.

==> Makefile <==
#
# $Id: Makefile 279 2008-01-27 16:19:38Z balaji $
#
# Copyright (C) 2006-2007, University of Chicago. All rights reserved.
#

HEADER = main
PICS = pics
BIB = bib
TEX = text

TARGETS: $(HEADER).pdf
.PHONY: all clean $(HEADER).pdf

tex_files = $(shell find $(TEX) -name '*.tex' -print)
bib_files = $(shell find $(BIB) -name '*.bib' -print)
pic_files = $(shell find $(PICS) \
		\( -name '*.eps' -print \) -or \( -name '*.epsi' -print \) \
		-or \( -name '*.ps' -print \) -or \( -name '*.png' -print \) \
		-or \( -name '*.fig' -print \) -or \( -name '*.pdf' -print \) \
	)

$(HEADER).pdf:
	@if test "`which rubber`" != "" ; then \
		TEXMFOUTPUT=`pwd` rubber -d -f -Wrefs -Wmisc $(HEADER) ; \
	else \
		pdflatex $(HEADER) | tee latex.out ; \
		bibtex $(HEADER); \
		touch .rebuild; \
		pdflatex $(HEADER) | tee latex.out; \
		pdflatex $(HEADER) | tee latex.out; \
		rm -f latex.out ; \
	fi

clean:
	@if test "`which rubber`" != "" ; then \
		rubber -d --clean $(HEADER) ; \
	else \
		find . \( -name '*.blg' -print \) -or \( -name '*.aux' -print \) -or \
			\( -name '*.bbl' -print \) -or \( -name '*~' -print \) -or \
			\( -name '*.lof' -print \) -or \( -name '*.lot' -print \) -or \
			\( -name '*.toc' -print \) | xargs rm -f; \
		rm -f $(HEADER).dvi $(HEADER).log $(HEADER).ps $(HEADER).pdf $(HEADER).out \
			_region_* TAGS ; \
	fi


==> text/evaluation.tex <==
\section{Experimental Evaluation and Analysis}
\label{sec:eval}
In this section, we experimentally evaluate the impact of IB resource
sharing on performance (communication throughput) and the usage
of communication resources (see \secref{sec:comm_resources} -- \aparna{fix link}) 
between independent threads across the different IB features using
the setup described in \secref{sec:setup}. For each IB resource, we
evaluate sharing across 16 threads. In the figures below, x-way
sharing means the resource of interest is being shared x ways. In other
words, two-way sharing means the resource is shared between two 
threads (eight instances of the shared resource), 16-way sharing means 
the resource is shared between 16 threads (one instance of the shared 
resource), and so on. Similarly, we define the values of
\postlist\ and \unsigs\ with respect to the threads. In the following graphs, 
we are interested in the change in throughput with
increasing sharing rather than the absolute throughput obtained by
using certain features. We start with the \naive\ endpoint
configuration (MPI everywhere) in a multithreading environment and
move down each level of resource sharing.
 
 
\subsection{Memory Buffer sharing}
\label{sec:bufsharingeval}

%=================================================================
\begin{figure}[htbp]
  \centering
  \begin{minipage}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/buf_sharing.pdf}
    \par(a)
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/buf_sharing_resusage.pdf}
    \par(b)
  \end{minipage}
  \caption{(a) Message rate and (b) communication resource usage with increasing
  	BUF sharing across 16 threads.}
  \label{fig:bufsharing}
\end{figure}
%=================================================================

\noindent \emph{\textbf{Performance.}} \figref{fig:bufsharing}(a) shows
the performance-impact of sharing the memory buffer across the
independent CTXs for each thread. The throughput decreases with
increasing BUF sharing. In other words, the increasing concurrent DMA
reads to the same memory address demonstrably hurts throughput.

To pinpoint the cause of this problem, we experiment with using
independent buffers that are on the same page with and without 64-byte
cache alignment. Without cache alignment, the 16 independent buffers
would be on the same cache line since each buffer is only 2
bytes. \figref{fig:bufsharingexp}(a) shows that concurrent DMA reads
to different addresses on the same cache line are detrimental. Also, the
total number of PCIe reads (measured using PMU tools~\cite{pmu_tools})
with and without cache alignment is the same. However,
\figref{fig:bufsharingexp}(b) shows that the rate of these PCIe reads
is much slower when the buffers are on the same cache line. This points us
to how the NIC translates virtual addresses (contained in the WQE)
to physical addresses needed for a DMA read of the payload, bolstering the analysis in
\secref{sec:bufsharing}. From our evaluation we can infer that the
hash function of the NIC's parallel TLB design is based on the cache
line, causing all translations to hit the same TLB with 16-way BUF
sharing.

\noindent \emph{\textbf{Resource usage.}} \figref{fig:bufsharing}(b) shows
that sharing the buffer has no impact on the usage of communication
resources.

%=================================================================
\begin{figure}[htbp]
  \centering
  \begin{minipage}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/buf_sharing_exp.pdf}
    \par(a)
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/pcie_rds.pdf}
    \par(b)
  \end{minipage}
  \caption{Effects on (a) message rate and (b) PCIe reads with and
    without cache-aligned buffers.}
  \label{fig:bufsharingexp}
\end{figure}
%=================================================================

\subsection{Device Context Sharing}
\label{sec:ctxsharingeval}

%=================================================================
\begin{figure}[htbp]
	\centering
	\begin{minipage}[t]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{pics/ctx_sharing.pdf}
		\par(a)
	\end{minipage}
	\begin{minipage}[t]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{pics/ctx_sharing_resusage.pdf}
		\par(b)
	\end{minipage}
	\caption{(a) Message rate and (b) communication resource usage with increasing
		CTX sharing across 16 threads.}
	\label{fig:ctxsharing}
\end{figure}
%=================================================================

With CTX sharing, the QPs of multiple threads are contained within
the same CTX.

\noindent \emph{\textbf{Performance.}} \figref{fig:ctxsharing}(a)
shows that sharing the CTX doesn't hurt performance for all
configurations except when we do not use \postlist\ \ie\ when
we use \blueflame\ writes. For example, we notice a 1.15x drop
in performance going from 8-way to 16-way CTX with maximally
independent TDs. While the engineers at Mellanox
Technologies are able to reproduce this drop even on the newer
ConnectX-5 card, the cause for the drop is unknown. We discovered
that creating twice the number of maximally independent TDs but
using only half of them (even or odd ones) can eliminate this drop, as
seen in the ``All w/o Postlist 2xQPs" line. Additionally, without our
patch, the Verbs user cannot request for maximally independent paths;
from the ``All w/o Postlist Sharing 2" line, we can see the harmful effects of
sharing a CTX when the mlx5 provider uses the second sharing level
(its default) for assigning TDs to uUARs. Again, while this evaluation
validates the need for maximally independent paths, it does not explain
the decline in throughput when there are concurrent \blueflame\ writes
to distinct uUARs sharing the same UAR page. Finding the precise reason
for this behavior is hard since the hardware-software interaction is
dependent on two proprietary technologies -- (1) the CPU architecture's
implementation of flushing write combining memory, which is used in
\blueflame\ writes, and (2) the NIC's ASIC logic that distinguishes between
a  \blueflame\ write and a \doorbell.

\noindent \emph{\textbf{Resource usage.}} \figref{fig:ctxsharing}(b)
shows that sharing the CTX does not impact QP and CQ usage but it 
greatly impacts uUAR and UAR usage. This is because a
maximally independent TD within a shared CTX adds only one UAR
as opposed to nine UARs when it is created within its own independent
CTX. Creating twice as many TDs to address the 8-way to 16-way
CTX sharing drop increases the number of QPs and UARs by 16,
and uUARs by 32 (``2xQPs" in \figref{fig:ctxsharing}(b))
since each of the extra 16 maximally independent TDs allocates its
own QP and UAR. On the other hand, the second level of sharing
that mlx5 is hardcoded to use consumes twice as low the number
of UARs as the default maximally independent TDs within a shared
CTX, resulting in eight and 16 lesser UARs and uUARs, respectively.

\subsection{Protection Domain Sharing}
\label{sec:pdsharingeval}

%=================================================================
\begin{figure}[htbp]
  \centering
  \begin{minipage}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/pd_sharing.pdf}
    \par(a)
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/pd_sharing_resusage.pdf}
    \par(b)
  \end{minipage}
  \caption{(a) Message rate and (b) communication resource usage with increasing
  	PD sharing across 16 threads.}
  \label{fig:pdsharing}
\end{figure}
%=================================================================

To study the impact of sharing protection domains, we fix the number
of CTXs to one because a PD cannot be shared across CTXs.

\noindent \emph{\textbf{Performance.}} From
\figref{fig:pdsharing}(a), we observe that sharing PDs across
the QPs of the threads has no effect on performance, supporting
our analysis in \secref{sec:pdsharing}.

\noindent \emph{\textbf{Resource usage.}} \figref{fig:pdsharing}(b)
shows that PD sharing has no effect on communication resource
usage either. The uUAR and UAR values reflect those of one CTX
containing 16 maximally independent TDs.

\subsection{Memory Region Sharing}
\label{sec:mrsharingeval}

%=================================================================
\begin{figure}[htbp]
  \centering
  \begin{minipage}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/mr_sharing.pdf}
    \par(a)
  \end{minipage}
  \begin{minipage}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/mr_sharing_resusage.pdf}
    \par(b)
  \end{minipage}
  \caption{(a) Message rate and (b) communication resource usage with increasing
  	MR sharing across 16 threads.}
  \label{fig:mrsharing}
\end{figure}

Since the memory region can be shared only under a PD, we set the
number of PDs and consequently the number of CTXs to one.
Keeping the BUFs independent for each thread, sharing
the MR implies that the MR spans multiple buffers, a situation that is
possible only if the BUFs of the threads are contiguous. Building on
our observations in \secref{sec:bufsharingeval}, we ensure that the
BUFs of each thread are cache aligned even though they lie in the same
contiguous memory area.

\noindent \emph{\textbf{Performance.}} \figref{fig:mrsharing}(a) shows
that sharing the MR between threads does not hurt throughput as long
as the memory buffers of each thread are cache-aligned, supporting our
analysis in \secref{sec:mrsharing}. If the buffers are not cache-aligned,
sharing the MR means sharing the buffer as well and we would observe
the same effect of BUF sharing as seen in \figref{fig:bufsharing}(a).

\noindent \emph{\textbf{Resource usage.}} \figref{fig:mrsharing}(b)
shows that sharing the MR does not impact communication resouce
usage.

\subsection{Completion Queue Sharing}
\label{sec:cqSharing}

%=================================================================
\begin{figure}[htbp]
	\centering
	\begin{minipage}[t]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{pics/cq_sharing.pdf}
		\par(a)
	\end{minipage}
	\begin{minipage}[t]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{pics/cq_sharing_resusage.pdf}
		\par(b)
	\end{minipage}
	\caption{(a) Message rate and (b) communication resource usage with increasing
		CQ sharing across 16 threads.}
	\label{fig:cqsharing}
\end{figure}
%=================================================================

A completion queue is associated only with the CTX and can be shared
only within a CTX. Therefore, we set the number of CTXs to one and keep
all the other resources independent between the 16 threads. For this
evaluation, we use the standard CQ instead of the extended CQ since
the lock on the CQ is needed for multithreaded access. With CQ
sharing, each CQ will contain completions for multiple QPs. Hence, we
multiply the CQ depth by x-way CQ sharing since the depth of the
CQ must be able to accommodate the maximum number of outstanding
completions. 

\noindent \emph{\textbf{Performance.}}
\figref{fig:cqsharing}(a) demonstrates that hurtful effects of CQ
sharing corresponding to the analysis in \secref{sec:cqsharing}.
In the ``All" and ``All w/o \blueflame" lines, we see a drop only
after 8-way sharing because there exists a tradeoff space between
the benefits of \unsigs\ and the overheads of CQ sharing.
\figref{fig:varyingunsig}(a) portrays this tradeoff space. Lower values
of \unsigs\ correspond to higher overheads, which are most visible in
``All w/o \unsigs" where every WQE generates a completion. For
different \unsig\ values, we see a drop in throughput
only after a certain level of CQ sharing because the benefits of
\postlist\ outweigh the impact of contention. When we remove the
benefits from \postlist, \figref{fig:varyingunsig}(b) shows a linear
decrease in throughput with increasing contention.

%=================================================================
\begin{figure}[htbp]
	\begin{center}
		\includegraphics[width=0.49\textwidth]{pics/varying_unsig_x_postlist_cqsharing.pdf}
	\end{center}
	\caption{(a) Postlist size of 32, (b) Postlist size of 1.}
	\label{fig:varyingunsig}
\end{figure}
%=================================================================

\noindent \emph{\textbf{Resource usage.}} \figref{fig:cqsharing}(b)
shows that sharing the CQ does not impact hardware resource usage.
However, it improves the total memory consumption of the software
communication resources by 1.1x with 16-way sharing.

\subsection{Queue Pair Sharing}
\label{sec:qpSharing}

%=================================================================
\begin{figure}[htbp]
	\centering
	\begin{minipage}[t]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{pics/qp_sharing.pdf}
		\par(a)
	\end{minipage}
	\begin{minipage}[t]{0.24\textwidth}
		\centering
		\includegraphics[width=\textwidth]{pics/qp_sharing_resusage.pdf}
		\par(b)
	\end{minipage}
	\caption{(a) Message rate and (b) communication resource usage with increasing
		QP sharing across 16 threads.}
	\label{fig:qpsharing}
\end{figure}
%=================================================================

The queue pair can be shared only within a PD. Hence, we set the
number of PDs and consequently the number of CTXs to one. For
this evaluation, we do not use TDs since the QP has to support
multithreaded access. Additionally, we use the standard CQ since
sharing a QP with its own CQ means sharing the CQ as well; hence,
requiring the need for a lock on the CQ.

\noindent \emph{\textbf{Performance.}}
\figref{fig:qpsharing}(a) reports throughput with increasing QP
sharing between 16 threads and supports the expected decline analyzed
in \secref{sec:qpsharing}. Similar to CQ sharing, the threads can
read each other's completions and hence require atomic updates
for their completion counters. Removing \postlist\ is more detrimental
than removing \unsig\ because we naturally expect more contention on
the QP's lock without \postlist.

\noindent \emph{\textbf{Resource usage.}}
\figref{fig:qpsharing}(b) shows that sharing the QP does not
impact hardware resource usage. The reason why the
absolute hardware resource usage of no QP sharing is
lower than that of no CQ sharing even though they both have
one CTX is because the CQ sharing evaluation uses dynamically
allocated uUARs and UARs with maximally independent TDs, unlike
this QP sharing evaluation which used the statically allocated uUARs
and UARs to allow for multithreaded access. QP sharing reduces both
the number of QPs and CQs, hence reducing the total memory
consumption of the software communication resources by 16x with
16 threads.


==> text/memandlimits.tex <==
\section{Resource Space and Limits}
\label{sec:memandlimits}

In \secref{sec:memusage} we detail the memory usage of the various
Verbs resources and the impact of resource sharing on memory usage. We
also study the limits of Verbs resources---the maximum number of
entities we can create for each Verbs resource---in
\secref{sec:reslimits}.

\subsection{Memory Usage}
\label{sec:memusage}

\tabref{tab:resmem} shows the memory used by each type of a Verbs
resource. We measure this memory usage manually using \texttt{gdb} on
MOFED4.1 by hitting breakpoints on \texttt{malloc}, \texttt{calloc},
\texttt{posix\_memalign}, and \texttt{mmap} during the corresponding
resource creation functions. Creating 1 endpoint requires at least 354
KB of memory, with the CTX occupying 74.2\% of it. Since the CTX is
the major consumer of an endpoint's memory and can be shared across
QPs, we next measure the total memory used for multiple endpoints with
and without CTX sharing. \figref{fig:memsharing}(a) shows an increase
of over 14x in memory usage going from 1 to 16 endpoints with distinct
resources for each endpoint. If we share CTXs between the endpoints,
we can reduce the memory footprint by up to 9x in the case of 16
endpoints according to \figref{fig:memsharing}(b). Note, however, that
any amount of CTX sharing, according to \secref{sec:ctxSharing}, will
impact performance. More important, both \tabref{tab:resmem} and
\figref{fig:memsharing} show that the absolute memory consumption of
the Verbs resources is minimal---on the order of megabytes---and thus
has barely noticeable impact on memory consumption. The memory on the
nodes of clusters and supercomputers is typically on the order of
hundreds of gigabytes. Hence, from a memory perspective, creating
distinct resources for each endpoint is viable.

\begin{table}
  \begin{center}
    \caption{Bytes used by Verbs resources} \label{tab:resmem}
    \begin{tabular}{  c | c | c | c | c | c }
      \hline
      \textbf{CTXs} & \textbf{PDs} & \textbf{MRs} & \textbf{QPs} & \textbf{CQs} 	& \textbf{Total} \\ \hline
      256K & 144 & 144 & 80K & 9K & 345K \\
      \hline
    \end{tabular}
  \end{center}
\end{table}
%GAIL - usually table captions go above the table, figure captions below

%=================================================================
\begin{figure}[htbp]
  %\vspace{-20pt}
  \centering
  %-----------------------------------------------------------------------------------------
  \begin{minipage}[t]{0.24\textwidth}\centering\includegraphics[width=\textwidth]{pics/memusage_nosharing.png}\par(a) 1 QP-per-CTX \end{minipage} 
  \begin{minipage}[t]{0.24\textwidth}\centering\includegraphics[width=\textwidth]{pics/memusage_ctxsharing.png}\par(b) CTX-sharing \end{minipage}
  %-----------------------------------------------------------------------------------------
  %\vspace{1em}
  \caption{Memory usage (in MB) of 16 endpoints.}
  \label{fig:memsharing}
  %\vspace{-1em}
\end{figure}
%=================================================================

\subsection{Resource Limits}
\label{sec:reslimits}

We primarily study the limits on the ConnectX-4 NIC, which is an mlx5
device. We programmatically attempt to hit the maximum number of
entities we can create for each resource. Our experimentally found
limits match those reported by MOFED-4.3's\footnote{The calculation of
  \texttt{max\_device\_ctx} is wrong in versions earlier than
  MOFED-4.3} \texttt{ibv\_devinfo} but with certain caveats. The
maximum number of CTXs (\texttt{max\_device\_ctx} field in
\texttt{ibv\_devinfo}) we can create is 1,021. The calculation of
1,021 assumes, rightly so, that each CTX contains 8 UAR pages since
MOFED's libmlx5 driver maps 8 UAR pages during
\texttt{ibv\_open\_device}. In OFED, on the other hand, we can control
the number of UAR pages mapped in a CTX through the MLX5\_TOTAL\_UUARS
environment variable. Setting it to 512 (2 times MLX5\_MAX\_UARS), we
can create a maximum of only 31 CTXs. Hence, the limit on CTXs is
imposed by the number of hardware registers (uUARs in Mellanox
terminology) available on the NIC. From the varying limit on CTXs, we
derive that the ConnectX-4 adapter hosts 16336 hardware registers (2
uUARs per 8,168 UARs).

The upper limit of the other resources is on the order of hundreds of
thousands and millions. For example, we can create 16 million CQs and
262,000 QPs across processes on a node with one ConnectX-4 HCA. Hence,
we are ultimately bottlenecked by the 16,000 hardware registers. This
take-away also holds for mlx4 devices such as the ConnectX-3 adapter
where we are limited by 8,088 Blue Flame registers and 1,011 regular
Doorbell registers; the maximum entities of the other resources is at
least a magnitude higher.

Thus, to create multiple endpoints on a node, we conclude that we will
run into hardware resource limits before running out of memory. These
limits hold beyond Mellanox adapters as well. Intel Omni-Path's HFI
adapter, for example, features 160 independent hardware
registers~\cite{opaUG}.


==> text/old_analysis.tex <==
\section{Resource Sharing Analysis}
\label{sec:analysis}

%=================================================================
\begin{figure*}[htbp]
  \centering
  \begin{minipage}[t]{0.26\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/ib_res_dep.pdf}
    \par(a)
  \end{minipage}
  \begin{minipage}[t]{0.70\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/mlx5_sharing.pdf}
    \par(b)
  \end{minipage}
  \caption{(a) Hierarchical relation between the various Verbs
    resources (the arrow points to the parent); each resource can have
    multiple children but only one parent. (b) Four levels of sharing
    in mlx5 between two independent threads.}
  \label{fig:sharinganalysis}
\end{figure*}
%=================================================================

In Mellanox InfiniBand, a thread can map to the hardware resource (uUAR) in four possible ways, each of which represents a level of
sharing with another thread.  \figref{fig:sharinganalysis}(b)
demonstrates the four ways described below. 
\begin{enumerate}
\item \emph{Maximum independence} -- No sharing of any hardware resource between the threads; each thread is assigned to its own UAR page (used in MPI everywhere).  
\item \emph{Shared UAR} -- The threads are assigned to distinct uUARs sharing the same UAR page (mlx5 default for multiple TDs described in \secref{sec:ctxsharing}).  
\item \emph{Shared uUAR} -- Although the threads have their own QPs, the distinct QPs share the same uUAR (regular uUARs in \secref{sec:ibresources}). A lock is needed on the shared uUAR for concurrent \blueflame\ writes. 
\item \emph{Shared QP} -- The threads share the same QP (used in state-of-the-art MPI+threads), in which case a lock on the QP is needed for concurrent device WQE preparation. The lock on the QP also protects concurrent \blueflame\ writes on the uUAR since the lock is released only after a \blueflame\ write.
\end{enumerate}


While sharing software and hardware communication resources at
different levels can improve resource efficiency, it can also hurt
throughput. Below, we explore the tradeoff space between resource
efficiency and communication throughput from the perspective of
Mellanox InfiniBand user while considering the various IB features
described in \secref{sec:ibfeatures}.  The user allocates the
interconnect's resources and interacts with them through the IB
resources shown in \figref{fig:sharinganalysis}(a).  Each of those
objects represents a level of sharing between independent threads. We
start with the \naive\ approach---each thread driving its own set of
resources---and then move down each level of IB resource sharing
according to the hierarchical relation in
\figref{fig:sharinganalysis}(a).

\subsection{Memory Buffer Sharing}
\label{sec:bufsharing}

The highest level of sharing is the non-IB resource: memory
buffer. The BUF refers to the memory location that contains the
payload of the message. We define the BUF to be the pointer to the
payload. If the payload size is small enough, it can be inlined within
the message descriptor. By default, the maximum message size that can
be inlined on ConnectX-4 exposed through Verbs is 60 bytes. Therefore,
for a message size larger than 60 bytes, the NIC must DMA-read the
payload through a memory region.

\noindent \emph{\textbf{Performance.}} When the payload cannot be
inlined, sharing this BUF between the threads' memory regions seems
harmless since the NIC will only ever read from it on the sender
node. However, the NIC's TLB design is important to consider since a
virtual-to-physical address translation is imperative for a DMA
read. The NIC typically has a multirail TLB design that handles
multiple transactions in parallel in order to sustain the high speed
of the NIC's ASIC. The load is distributed across the TLBs by using a
hash function. If this hash function is based on the cache line,
concurrent DMA reads to the same cache line will hit the same
translation engine, serializing the reads. With a shared BUF, the WQEs
of multiple threads would point to the same cache line and serialize
the DMA reads. When the payload can be inlined, however, sharing the
BUF is harmless since the CPU reads the payload instead of the
NIC. Concurrent reads to the same memory location in a CPU are
harmless.

\noindent \emph{\textbf{Resource usage.}} Sharing the BUF reduces
memory usage. However, its impact on memory consumption is
proportional to the size of the payload of the message. It doesn't
affect the usage of any of the communication resources.

\subsection{Device Context Sharing}
\label{sec:ctxsharing}

The highest level of sharing among the IB resources is the device
context. This is essentially a container of hardware and software
resources that the other IB resources within the CTX will use.  These
hardware resources are either statically allocated during CTX creation
or dynamically allocated when the user uses hints such as thread
domains (see \secref{sec:ibresources}).

Sharing a CTX between threads means that the CTX contains multiple
QPs. These multiple QPs may or may not share the hardware resources
contained within the context. Even if multiple QPs are assigned to
distinct uUARs, the uUARs could share the same UAR page.  Without CTX
sharing, this is never the case since the QPs naturally get assigned
to uUARs on different UAR pages.

More important, the Verbs user has no way to explicitly request
maximally independent paths. When the user creates multiple TDs, the
mlx5 provider can assign the threads to a uUAR using either the first
or the second level of sharing, as shown in
\figref{fig:sharinganalysis}(b); the third and fourth levels of
sharing do not apply to TDs since they imply multithreaded access to one
hardware resource. Currently, the mlx5 provider is hardcoded to use
the second level of sharing for multiple TDs, restricting the user
from creating maximally independent QPs within a CTX. More abstractly,
the Verbs users today have no way to request for a sharing level for
the QPs/TDs they create. The number of levels of sharing is provider
specific, and one can imagine multiple levels of sharing to exist for
TDs.

To overcome this Verbs design limitation, we propose a variable,
\texttt{sharing}, in the TD initialization attributes (\texttt{struct
  ibv\_td\_init\_attr}) that are passed during TD creation. The higher
the value of \texttt{sharing}, the higher is the amount of hardware
resource sharing between multiple TDs. A \texttt{sharing} value of $1$
refers to maximally independent paths. In mlx5, only two levels of
sharing exist for TDs, corresponding to (1) and (2) in
\figref{fig:sharinganalysis}(b).

Note that the second uUAR of the UAR dedicated to a maximally
independent TD is wasted. Since the number of hardware resources is
limited, the user can request only a certain maximum number of
independent hardware resources within a CTX. This would be half of the
maximum number of UARs the user can dynamically allocate using TDs. In
mlx5, the maximum number of maximally independent paths is 256.

\noindent \emph{\textbf{Performance.}} For maximally independent
threads, sharing the CTX should not affect performance since we
emulate the QP-to-uUAR mapping of endpoints in the MPI everywhere
model, which represents the maximum possible throughput for a given
number of threads. Sharing a CTX with the second level of sharing
between independent threads could hurt performance. The NIC could
implement its mechanism of reading concurrent \doorbells\ and
\blueflame\ writes at the granularity of UAR pages, negatively
impacting throughput when multiple QPs are assigned to uUARs on the
same UAR page. The CPU architecture's implementation of flushing write
combining memory can also impact performance in the second level of
sharing since the memory attribute of the uUARs is set at the page
level granularity using the Page Attribute Table (PAT)~\cite{pat}.

\noindent \emph{\textbf{Resource usage.}} Sharing the CTX is critically
useful for both memory consumption and uUAR usage. For example, when 
shared between 16 threads, it can reduce the memory consumption by 9x
(reducing from 5.15 MB to 0.35 MB).  More important, sharing the CTX
means that the 16 static uUARs allocated by the mlx5 provider during
CTX creation (see \secref{sec:ibresources}) are wasted only
once. Nonetheless, maximally independent threads will waste one uUAR
per thread. On the other hand, sharing the CTX with the second level
of sharing will not waste any uUAR after the 16 static ones.

\subsection{Protection Domain Sharing}
\label{sec:pdsharing}

The next level of sharing between threads is the protection
domain. The PD is a means of isolating a collection of IB
resources. Resources such as QPs and MRs contained under different PDs
cannot interact with each other. For example, a QP on the sender node
cannot access a remote MR on the receiver node owned by a PD that does
not contain the receiver QP connected to the sender QP.

\noindent \emph{\textbf{Performance.}} The software PD object is not
accessed on the critical data-path; the protection checks occur in the
NIC. Hence, from a performance perspective, sharing a PD between
multiple threads would be harmless.

\noindent \emph{\textbf{Resource usage.}} Sharing the PD between
threads will reduce memory consumption but only marginally so since
each PD occupies less than 200 bytes. The PD doesn't impact the usage
of any of the communication resources.


\subsection{Memory Region Sharing}
\label{sec:mrsharing}

Within a protection domain, the memory region can be shared between
multiple threads. The MR is an object that registers a region in the
virtual address space of the user with the operating
system. Registering a memory region means pinning the memory and
preparing that region for DMA accesses from the NIC. The virtual
address region typically corresponds to that of the memory buffer. The
MR is a precondition for when the NIC needs to access a node's (local
or remote) memory.

\noindent \emph{\textbf{Performance.}} Sharing the MR itself between
threads will have no impact on performance since the MR is just an
object that points to a registered memory region. The MR may span
multiple BUFs given that they are contiguous. Sharing an MR that
contains only one BUF means the threads are sharing the BUF as well,
which would imply the same effects of BUF sharing when the
payload cannot be inlined for an operation that sends data over the
wire such as an RDMA write.

\noindent \emph{\textbf{Resource usage.}} Sharing the MR between
threads will reduce memory consumption but only marginally so since,
like the PD, each MR occupies less than 200 bytes. The MR doesn't
impact the usage of any of the communication resources.


\subsection{Completion Queue Sharing}
\label{sec:cqsharing}

The completion queue is a work queue that contains completion queue
entries corresponding to the successful or unsuccessful completion of
the WQEs posted in the QP. The user actively polls the CQ on the
critical data-path to confirm progress in communication. The IB
specification guarantees ordering between the completions; that is, a
successful poll of the $n$th WQE guarantees the completion of all the
WQEs prior to it. The Verbs user can map multiple QPs to the same CQ.

\noindent \emph{\textbf{Performance.}} The CQ has a lock that a thread
will acquire before polling it. Hence, the threads sharing a CQ will
contend on its lock. Additionally, if QP $i$ and QP $j$ share a CQ,
then thread $i$ driving QP $i$ could read QP $j$'s completions. Hence,
the completion counter for any thread $i$ requires atomic updates.
The atomics and locks are obvious sources of contention when sharing
CQs between threads. Additionally, lower values of \unsigs\ imply that
the thread reads more completions from the CQ than for higher values.
This translates to the thread currently polling the shared CQ holding
the lock longer than it needs to, in order to read fewer
completions. Thus, the impact of lock contention on the shared CQ is
higher without \unsigs\ than with. The user may use \unsigs\ if the
semantics of the user's application allows that.

Even if the Verbs user can guarantee single-thread access to a CQ, the
standard CQ does not allow the user to disable the lock on the CQ. The
extended CQ, on the other hand, allows the user to do so during CQ
creation (\texttt{ibv\_create\_cq\_ex}) with the
\texttt{IBV\_CREATE\_CQ\_ATTR\_SINGLE\_THREADED} flag.

\noindent \emph{\textbf{Resource usage.}} Sharing the CQ translates to
lesser circular buffers and hence it reduces memory consumption of the
completion communication resource.


\subsection{Queue Pair Sharing}
\label{sec:qpsharing}

Ultimately, the user can choose to share the queue pair between
threads to achieve maximum resource efficiency. This is the case in
state-of-the-art MPI implementations.

\noindent \emph{\textbf{Performance.}} The QP has a lock that a thread
needs to acquire before posting on it. Hence, threads will contend on a
shared QP's lock. Additionally, the threads need to coordinate to post
on the finite QP-depth of the shared QP since the values of
\postlist\ and \unsig\ are with respect to each thread. This
coordination requires atomic fetch and subtracts on the remaining
QP-depth value. The locks and atomics are obvious sources of
contention when sharing QPs between threads. Most important, the NIC's
parallel capabilities are not utilized with shared QPs since each QP
is assigned to only one hardware resource through which the messages
of multiple threads are serialized.

When the user assigns a QP to a thread domain, however, the lock on
the QP is still obtained. The mlx5 provider currently optimizes the
critical data-path by removing the lock only on the uUAR that the TD
is assigned to. Since the user guarantees no concurrent access from
multiple threads to a QP assigned to a TD, the lock on the QP itself
can be disabled. We optimize the mlx5 provider for this case by first
implementing the infrastructure to control locking on each individual
mlx5 Verbs object and then using it to disable the lock on a QP
assigned to a TD~\cite{mlx5lockcontrol}.

\noindent \emph{\textbf{Resource usage.}} Sharing the QP means lesser
circular buffers for the WQEs and hence, a lower memory
consumption. In the extreme case of one shared QP, we have only one of
each of the IB resources, resulting in minimum memory
usage. Furthermore, a shared QP between threads means only 15, as
opposed to 16 with a TD-assigned-QP per thread, static uUARs are
wasted. The 16th, low-latency uUAR is assigned to the shared QP.

